Crowdsourced Fact-Checking at Twitter: How Does the Crowd Compare With Experts?

Fact-checking is one of the effective solutions in fighting online misinformation. However, traditional fact-checking is a process requiring scarce expert human resources, and thus does not scale well on social media because of the continuous flow of new content to be checked. Methods based on crowdsourcing have been proposed to tackle this challenge, as they can scale with a smaller cost, but, while they have shown to be feasible, have always been studied in controlled environments. In this work, we study the first large-scale effort of crowdsourced fact-checking deployed in practice, started by Twitter with the Birdwatch program. Our analysis shows that crowdsourcing may be an effective fact-checking strategy in some settings, even comparable to results obtained by human experts, but does not lead to consistent, actionable results in others. We processed 11.9k tweets verified by the Birdwatch program and report empirical evidence of i) differences in how the crowd and experts select content to be fact-checked, ii) how the crowd and the experts retrieve different resources to fact-check, and iii) the edge the crowd shows in fact-checking scalability and efficiency as compared to expert checkers.

==> BirdWatch analysis/background.tex <==
%\vspace{-0.2cm}
\section{Background and Related Work}
\label{sec:relatedWork}

% \paolo{Gianluca, those are relevant papers that we should cite across the section - we need to stress that in previous work the crowd was in controlled environment - can you place them as you see fit?}
% \begin{itemize}
% \item Crowd quality, controlled environment, impact of bias/background (\cite{10.1145/3397271.3401112}) %sigir2020
% \item COVID claims, crowd quality, controlled environment, impact bias/background (\cite{10.1145/3340531.3412048}) %cikm-covid
% \item 
% The Role of the Crowd in Countering Misinformation: A Case Study of the COVID-19 Infodemic
% (\cite{9377956})
% \end{itemize}


Fact-checking requires a chain of steps that starts with identifying check-worthy claims and ends with a label about the veracity of the claim. Labels vary across services but usually can be divided into four popular categories: true, partially-true, false, or not enough evidence to judge. The top of Figure~\ref{fig:overview} shows a generic high-level fact-checking pipeline~\cite{nakov2021automated}. The three considered checking methods are then reported, specifically automatic methods, \BW crowd, and expert fact-checkers. Given an input textual tweet, every method can be used to assess if it is worth checking and eventually verified. For every checking method, we also report the dimensions that can be used to compare and contrast the alternative methods. 
%  
We discuss next the main steps in the pipeline, \rev{their related work}, and their implementation in the different methods.


%\vspace{1ex}
\textbf{Claim Selection.}
For claim selection we can use automatic methods, the crowd, or experts.
% 
Given a sentence, an automatic method scores if it contains check-worthy factual claims~\cite{HassanALT17,clef-checkthat-T1:2019,10.1145/3308560.3316736}. A model trained on annotated sentences gives low scores to non-factual and subjective sentences.
%
Deciding whether a claim is worth checking is similar to the task of judging the relevance of a document w.r.t. a search query. In Information Retrieval evaluation, well-trained experts (e.g., NIST assessors) may be used to produce judgements of relevance following guidelines, or be instead substituted by crowd workers who receive simple instructions. % and complete the task in limited time.
Similarly, check-worthiness may be performed by a panel of experts %following a formal process 
or crowdsourced, like done in \BW.
The crowdsourced annotation of textual content on social networks is a widely supported activity across all platforms. Users label content that violates the guidelines of the site, such as hate speech and misinformation. This process triggers the human verification with moderators hired by the platform~\cite{FacebookProgram,10.1145/3404835.3464926}. For expert, human fact-checkers the selection of the claims to verify is driven by journalistic principles, e.g., claims should contain \textit{verifiable} facts~\cite{TruthOMeter}.
Experts also assess if a claim is \textit{important}, with a definition that changes according to the public and the mission of the organization, e.g., voters and elections~\cite{WaPost}.
% \gd{maybe here I can write something about how this relates to relevance judgements where you usually have trained human assessors that follow a long set of instructions, or the crowd?}\paolo{sure, but i also remember you mentioned this paper where you show that they go after claim review and then you removed such pages in an ad-hoc search engine to see what else they pick}\gd{discussed below at the evidence retrieval step}
The crowd may have different criteria and priorities in deciding which claims to fact-check and a  definition of check-worthiness that takes into account the topic, the timeliness, and their own personal points of view. Previous research in crowdsourced fact-checking (e.g., \cite{8791903}) has not looked in detail at how the crowd may perform this step of the pipeline, and it is something that instead we do in this work.
% 


\begin{figure*}[t]
%\hspace{-2ex}
\includegraphics[scale=0.46]{images/example_bw.png}
\caption{\BW note and \CR fact-check Example. (A) shows a tweet. (B) is the note with the assigned label to such tweet. (C) is a sample of questions when submitting a note. (D) is a sample of questions when submitting a rating. (E) shows a fact-check delivered by an expert.}
%\vspace{-1ex}
\label{fig:bw_example}
%\vspace{-1ex}
\end{figure*}

%\vspace{1ex}
\textbf{Evidence Retrieval.}
For computational methods, we distinguish the task of detecting previously fact-checked claims and the task of gathering evidence to support the verification step. As false claims are often repeated across platforms and over time, independently of  available fact-checks, claim matching aims at automatically identifying an existing debunking article for the claim at hand~\cite{adler2019,ShaarBMN20,botnevik2020brenda}. Claim matching is feasible at scale because websites use the schema.org standard \CR metadata
  to share their checks~\cite{CRProject}.
For fresh claims, which have not been debunked yet, several methods aim at finding external evidence to help  fact-checkers and computational methods deciding on the veracity of a claim~\cite{thorne-etal-2018-fact}. The output is usually a ranking of  retrieved documents or specific passages~\cite{Alshomary:20}.
The crowd makes use of expert fact-checking outcomes when available. Indeed, \citet{roitero2020can} removed expert outcomes from the search results used by the crowd in their fact-checking task to avoid influencing crowd worker judgments.
Expert fact-checkers instead rely on their training to identify proven, verified, transparent, and accountable evidence~\cite{evaluate}, sometimes involving third-party domain experts~\cite{fffaq}. %\footnote{\url{https://fullfact.org/about/frequently-asked-questions/}}.



%\vspace{1ex}
\textbf{Claim verification.} A large body of research focus on developing and evaluating automatic solutions for fact-checking \cite{nakov2021automated,vo2018rise,BrandRSD21,botnevik2020brenda,10.1145/3404835.3463120,10.1145/3331184.3331305,Karagiannis0PT20}. However, there are coverage and quality issues with automated systems~\cite{fullfact:coof}, and thus a pragmatic approach is to build tools to facilitate human fact-checkers
%, such as tools to steer human checkers with url recommendation
~\cite{vo2018rise}.  At the same time, effort in artificially creating rumors and misinformation has been shown to be effective \cite{huynh2021argh}.
The crowd makes use of evidence from the Web and is influenced by their own personal belief and context \cite{10.1145/3340531.3412048,DBLP:conf/ecir/BarberaRDMS20}. Interestingly, when misinformation is identified on social media, users tend to counter it by providing evidence of it being misleading 
\cite{9377956}. This shows an intrinsic motivation that certain members of the crowd have to contribute to the checking process.
An approach for crowd-sourced fact-checking is using tools that surface relevant evidence for their judgement \cite{fan2020generating}. This however comes with the risk of over relying on such tools to make judgements  \cite{10.1145/3242587.3242666}.
% Most expert fact-checkers work within organizations that are part of the International Fact-Checking Network, which sets editorial standards on the verification protocol\footnote{\url{https://www.poynter.org/ifcn-fact-checkers-code-of-principles/}}.
%It can take either the full page opened in the browser or a highlighted snippet inside the page. In the first scenario, the system applies check-worthiness identification in order to decide which sentences to fact-check.  

Finally, there has been some early analysis of the \BW data~\cite{allen_martel_rand_2021,Prollochs2021CommunityBasedFO}, but they focus only on the tweets and notes content, while we rely on the manually aligned expert claim reviews to compare \BW results against the best solution in this space.
A related study has looked at a Reddit community involved in the fact-checking process using a crowdsourced approach \cite{10.1145/3308560.3316734}. %It shows potential for an hybrid crowd, experts, and systems solution to the problem.




==> BirdWatch analysis/conclusion.tex <==

\section{Discussion}
\label{sec:discussion}
% From our study, there are at least three main topics that are worth highlighting.

\subsection{Collaborative solutions}
The analysis of the quality of the \BW users 
%for claim selection, evidence retrieval, and claim verification 
shows that crowdsourced fact-checking is a promising and complementary solution, with results that correlate with those of professional fact-checkers. However, we argue that a crowd-based solution should not be considered to replace experts, but rather as a tool in collaborative effort where, for example, the crowd helps flagging content and creating links to more sources of trustable evidence. Indeed, our results show that the crowd can be even more reactive than experts to a new false claim and is able to identify a large array of high quality sources of evidence. This is especially important, as there is evidence that fact-checking interventions are significantly more effective in novel news situations~\cite{Nevo2022}.

Looking forward, and assuming we can characterize the trust and the cost level for all involved actors (i.e., crowd, experts, and computational methods), there is an opportunity to design novel hybrid human-machine solutions that coordinate this joint effort in order to combine the benefits of the different approaches. The role of automatic tools can be that of providing real-time and scalable fact-checking for all posted content. Platform users can then intervene quickly in a more focused manner to provide a first line of defense on potentially harmful content. This can then be followed by quality in every step of the fact-checking pipeline, with humans collectively processing evidence for the final labeling. 

\subsection{Hard to verify claims}
The matching process of tweets and claim-review checks led us to recognize the difficulty of this task. % for multiple reasons. 
The first challenge is %of course 
the semantic match in terms of content, but in many cases where the match is clear, the problem is hard even for humans. Several problems, such as sarcasm and vagueness, are known in general for the detection of worth-checking claims~\cite{clef-checkthat-T1:2019}. However, another problem is the granularity of the tweet. Even a very short tweet may contain two interleaved claims, such as ``Mike said: the earth is flat'' (see also, e.g., Tweet \#3 in Table \ref{tab:examples}). Assume there are two claim reviews, one checks that Mike made a claim about the earth (labeling the matching tweet as true), and the other checks about the fact that the planet is not flat (labeling the tweet as false).

This suggests the challenge of being able to identify the textual claims where both crowdsourcing and computational fact-checking methods are most likely to fail short. This can be modeled as a new supervised classification task aiming at predicting when a claim cannot be verified effectively without experts. 
{As an orthogonal approach, this is also an opportunity for automatic controversy detection methods (e.g., \cite{10.1145/2911451.2914745}) to play a complementary role in supporting the crowd, making them aware of potential controversies during their verification tasks.} 
%The task of detecting ``hard claims'' is especially important in the vision of enabling collaboration among the different methods, %  and finally present a model that can recognize the ``difficult'' claims,
%so that at verification time it may be possible to dynamically assign a claim based on its difficulty either to the automatic method, to the crowd, or to the expert checkers.
%\mohammed{hard to control social media}

\subsection{Stale claims}
We found clear evidence that claims that have been already verified by expert checkers keep circulating and spreading on Twitter, even months after the publication of their debunking~\cite{shin2017}.
Unfortunately, we have also observed that automatic methods still fail short in matching with high accuracy tweets that contain such ``stale" claims{, likely because of the peculiar language used in tweets.}
In such a setting, %it seems clear that 
\BW users can play an important role in quickly and effectively recognizing these cases.
% 
Indeed, the significant difference in the health-related \BW notes and \CR fact-checks is explained by the increase of tweets spreading already fact-checked claims.
% 
Stale claims are a good fit for the role of \BW participants, especially when automatic matching methods~\cite{ShaarBMN20,AhmadICDE} fail, while fresh claims might require proper forensic processes and need the expertise of journalists. %This way, expert fact-checkers and the crowd can complement each other to address the vast and growing amount of misinformation on social media.
%, where fact-checkers can verify the fresh claims effectively, and the crowd can combat the stale claims by propagating the fact-checks, even during the surge of false news such as those related to COVID.

\section{Conclusion}
\label{sec:conclusion}
In this paper, we present a data-driven analysis of the \BW program through the lens of the three main components of a fact-checking pipeline: claim detection based on check-worthiness, evidence retrieval, and claim verification. This is also the first study that bridges real data from a large-scale crowdsourced fact-checking initiative with the debunking articles produced by professional fact-checkers. \cam{While our analysis has been limited to \BW participants from the US, we hope the \BW initiative can be deployed globally for a more comprehensive analysis.}

Our study shows that 
%community-created 
\BW notes are effective in terms of claim verification, with encouraging results, in contrast with the negative results obtained by previous crowdsourcing efforts%, such as TruthSquad and WikiTribune
~\cite{BhuiyanZSM20}. However, we also show that in \BW a group of users sharing a common goal could potentially steer the final classification label, such as in the case of source credibility. This suggests that more attention is needed in identifying harmful groups by profiling their activity and by incorporating their biases in the note ranking system. Another approach would be to calibrate the selection of \BW participants to enforce high diversity %in the attempt 
to mitigate this issue~\cite{EpsteinPR20}.


Our results indicate  that the \BW program is a viable initial approach towards crowd-based fact-checking, which can help complement the work of expert fact-checkers.% by debunking misinformation on Twitter. %by the use of already available fact-checks. 
An interesting open question is how to develop a collaborative platform involving the different fact-checking methods (crowd-based, computational, and experts). 
Given different trust and cost profiles for the different methods, a model to assess the difficulty of validating a claim (either data-driven  or crowd-driven as in \BW), and a certain budget, what is the optimal way to assign the claim to each fact-checking method so that the number of verified claims is maximized with a high level of trust?

% Given a profile with trust and cost for the different checking methods, a model to characterize the hardness of a claim, and a budget, how to assign tasks to maximize the number of verified claims with a certain level of trust?


%\gd{sometimes we write `fact check*' and sometimes `fact-check*', make a pass at the end.}\paolo{i suggest to stick to fact-check} \mohammed{should be consistent now}

==> BirdWatch analysis/data.tex <==
\section{Data}
\label{sec:data}
Community-driven fact-checking on Twitter is governed by the \BW initiative~\cite{BWPublish}, while fact-checks written by journalists and expert fact-checkers are curated using the \CR schema~\cite{CRProject}. In this section, we describe both datasets and how to match similar claims identified by both parties. Approval from authors' institution research ethics committee to perform this study has been obtained prior to commencing.

\subsection{\BW}
\label{subsec:birdwatch}
Misinformation on Twitter can be mitigated through the \BW program, where participants can identify misleading tweets and provide more context~\cite{BWPublish}. Currently, \BW is only available to participants in the US, where users can identify misleading information using two core elements: \textit{Notes} and \textit{Ratings}.

{\textbf{Notes.}} Participants in the \BW program can add notes to any tweet. Their notes are formed from: (i) a classification label indicating whether the tweet is misinformed/misleading (\textbf{MM}) or not misleading (\textbf{NM}) according to their judgement, (ii) answers to several multiple-choice questions about their decision~\cite{BWdata},
%shown in Table~\ref{tab:note_questions}, 
and
%about the tweet such as whether it contains  outdated information, is a satire, or contains trustworthy sources, and 
(iii) an open text field where participants can justify their choice of the label and possibly include links to sources that prove their point. 
%Any participant could provide a note (or more) on any tweet. 
An example of a note is shown in Figure~\ref{fig:bw_example} (B,C). The key data we use from the notes are the following:
\begin{itemize}
    \item \textit{Classification Label}: Whether the tweet is %misleading/
    misinformed (MM) or not (NM) according to the \BW user (Section~\ref{subsec:ClaimVerif}).
    \item \textit{Note Text}: the text given by the user with the justification for the label (Sections ~\ref{subsec:topics} and \ref{subsec:rq1}).
    \item \textit{Timestamps}: time at which the note was written \rev{(Section~\ref{subsec:rq1}}).
\end{itemize}
%A participant could provide more than one note per tweet.\\
% \paolo{I think we need an example of the note and tweet pair, with at least a sample of the answers to the questions and sources}

{\textbf{Ratings.}} Participants rate the notes of other participants. Ratings help identify which notes are most helpful.
%, and allow \BW to raise the visibility of those found most helpful by a wide range of contributors. 
A user rates a note by providing answers to a list of questions~\cite{BWdata}. An example of a rating is shown in Figure~\ref{fig:bw_example} (D).
%\paolo{Missing ref to figure2, also a letter missing them - careful as adding it will change also D and E later}
%shown in Table~\ref{tab:rating_questions} \gd{broken ref}. 
Out of these questions, we focus on the following:
\begin{itemize}
    \item \textit{High-quality Sources:} The user answers the yes/no question `Is this note helpful because it cites high-quality sources?'. We use this information to assess whether \BW users distinguish credible sources~(Section \ref{sec:sourceQuality}).
    \item \textit{Helpfulness Label:} The user answers the question `Is this note helpful?'. The possible answers are (i) not helpful, (ii) somewhat helpful, and (iii) helpful. We use this information to compute an helpfulness score for notes (Section~\ref{subsec:ClaimVerif}).
\end{itemize}
% (i) agreeing/disagreeing with the note and (ii) providing answers to multiple choice questions including whether the note addresses the tweet's claim, if it has missing or unreliable sources, and if it was helpful or not. An example of questions for a rating is shown in Figure~\ref{fig:bw_example} (D).
%There are no open-text fields for ratings. 

All \BW notes start with a `Needs More Rating' status until enough ratings are achieved according to a platform defined threshold (currently set to 5). Once achieved, these ratings are aggregated and weighted by a `Rater Score' to compute the `Note Helpfulness Score'. A higher rater score gives more weight to participants (i) whose notes are found helpful by other participants, and (ii) whose ratings align with the final rating outcome. A higher note helpfulness score means that many participants found a note adequate, and it would likely hold a valid classification label. %Rating aggregation is visualized in Figure~\ref{fig:bw_example} (E).


\begin{figure}[h]
    \centering
    \pgfplotstableread[col sep=comma,]{files/Notes.csv}\datatable
    \begin{tikzpicture}[scale=0.9]
    \begin{axis}[
    	ymode=log,
	log basis y={10},
        ybar,
        xlabel={Number of Notes},
        xtick=data,
        xticklabels from table={\datatable}{NumNotes},
        ylabel={\# of Tweets},
        ymajorgrids,
        height=3cm,
        width=\columnwidth]
        \addplot table [x expr=\coordindex, y={Count}]{\datatable};
    \end{axis}
    \end{tikzpicture} 
    %\vspace{-2ex}
    \caption{Bar plot of the number of notes per tweet.}
       %\vspace{-1ex}
    \label{fig:BarNotes}

\end{figure}
\begin{figure}[h]
    \centering
    \pgfplotstableread[col sep=comma,]{files/NumRate.csv}\datatable
    \begin{tikzpicture}[scale=0.9]
    \begin{axis}[
        ybar,
        xlabel={Number of Ratings},
        xtick=data,
        xticklabels from table={\datatable}{NumRating},
        ylabel={\# of Notes},
        ymajorgrids,
        height=3cm,
        width=\columnwidth]
        \addplot table [x expr=\coordindex, y={Count}]{\datatable};
    \end{axis}
    \end{tikzpicture}
    %\vspace{-1ex}
    \caption{Bar plot of the number of ratings per note.}
    \label{fig:BarRates}
\end{figure}

{\textbf{Descriptive Statistics.}} We use the \BW data up to September 18$^{th}$ 2021. The dataset contains 86,924 ratings for 15,445 notes on 11,871 tweets from 5124 unique \BW participants. Bar plots of the number of notes and ratings are shown in Figure \ref{fig:BarNotes} and Figure~\ref{fig:BarRates}, respectively. Most tweets have only one or two notes, while
%indicating the need for more notes for a higher note score. T
the tweet with the most notes has 61. The majority of notes have less than five ratings, and the most rated note has 184 ratings. The user with most notes checked 656 tweets with around 71\% related to US Politics. %saving a line: , and the rest to COVID-19. 
Among these 656 tweets, 643 do not have any other note. The user with most notes in common with other users shares 85 notes (on 85 tweets) with 217 other users. %This user’s labels agree with other users' classifications in 68/85 tweets.

\subsection{\CR}
\label{subsec:ClaimReview}
The \CR project~\cite{CRProject} is a schema used to publish fact-checking articles by organizations and journalists. The schema defines % schema.org
mark-up tags that are used in web pages so that search engines identify the  information in a debunking article, such as text claim, claim label, and author~\cite{CRSchema}.
Our dataset is a collection of items following the \CR schema, collected from various sources %and processed to obtain ratings about several entities, such as Tweets
%, URLs, web domains  and news outlets
\cite{MensioA19}. Each item, or \textit{fact-check}, is a (claim, label) pair produced by a professional journalist or fact-checking agency.
\rev{We assume that professional fact-checkers do not overlap with \BW participants, as the former have no interest in doing their work without retribution.}
Since different fact-checkers use different labels, the data is normalized into a smaller subset of labels (credible, mostly credible, uncertain, unverifiable, not credible). In addition to the claim and the label, the checks also contain a link to the fact-checking article. % and the list of URLs where the claim appears. 
Note that checked claims in this dataset could occur anywhere on the web and need not be only on Twitter.
We use a dataset containing 76,769 fact-checks. %ranging till the 19th of April 2021. 
Examples of the data are shown in Figure~\ref{fig:bw_example} (E) and Table~\ref{tab:examples}.

\subsection{Matched Data}
\label{subsec: MatchedData}
To study how the judgements of the crowd compare to those of expert fact-checkers, we match claims from both datasets. %by relying on an unsupervised text-to-text matching algorithm~\cite{ShaarBMN20} to pair the text of the tweet to that of the claim in \CR fact-checks.
%to match claims of both datasets. 
\rev{As the automatic matching is imperfect, we used the Amazon Mechanical Turk crowdsourcing platform~\cite{AMTurk} for matching the text in the tweets checked by the \BW crowd with the claim text in the \CR fact-checks. When workers accepted a Human Intelligence Task (HIT), they were shown (i) the tweet that is to be matched and (ii) the top-10 similar \CR checks provided by SentenceBERT using a bi-encoder with cosine similarity \cam{between the text of the tweet and that of the claim in \CR fact-checks}~\cite{reimers-gurevych-2019-sentence}. We also add a `None of the Above' option for cases where the worker could not find a match.
A manual inspection of the matches showed that the vast majority of tweets with a score below 0.6 do not have matching \CR checks. We therefore run the annotation for tweets with at least 0.6 as top-1 similarity score. The workers were required to have at least 500 approved HITs to access our task, which comprised of 5322 tweets to be matched. Each tweet was shown to 3 workers\cam{, similar to previous work~\cite{Kazai2011,Du2012}.} %and every worker was awarded \$0.1 for completed HIT.
\cam{The hourly rate based on median completion time was 12.41\$.}
}

%manually label the 500 tweets with top similarity scores against \CR fact-checks according to the algorithm. The labelling was done with 5 annotators, each being trained on \BW and \CR data, where each annotator had 30\% of their data in common with other annotators to compute inter-annotator agreement. Annotators were given a list of tweets and the top 200 fact-check matches for each tweet by the matching algorithm. The annotators marked whether at least one \CR matched the tweet text. 


\begin{figure}[t]
\pgfplotstableread[col sep=comma,]{files/TopicBar.csv}\datatable
\begin{tikzpicture}
\begin{axis}[
	ymode=log,
	log basis y={10},
    height=3cm,
    width=0.9\columnwidth,
    ymajorgrids,
	ylabel=Count,
	legend pos=outer north east,
	%xlabel=Topic,
	%legend style={at={(0.2,9.2)}
	%anchor=east},
	enlargelimits=0.1,
	ybar,
	bar width=4pt,
	xtick=data,
	xticklabels from table={\datatable}{Topic},
	x tick label style={rotate=30,anchor=east}],
]
\addplot
     table[x expr=\coordindex,y=BirdWatch]{\datatable};
\addplot
     table[x expr=\coordindex,y=Claim Review]{\datatable};

\legend{BW,CR}
\end{axis}
\end{tikzpicture}
%\vspace{-4ex}
\caption{Bar plot of tweets checked by \BW (BW) and \CR (CR) fact-checks for 2021 divided by topic.}
\label{fig:2021_topics}
%\vspace{-2ex}
\end{figure}


\begin{figure*}[t]
\includegraphics[scale=0.35]{images/TopicPlots.png}
%\vspace{-3ex}
\caption{Per-topic frequency histograms and KDE Plots for \BW (BW) notes and \CR (CR) fact-checks (month granularity).}
\label{fig:TopicPlot}
\end{figure*}

\rev{To measure the quality of the worker annotations, we manually annotated the top-500 tweets in terms of matching score. %that were had the top similarity scores according to a different matching algorithm than the one used for the workers.
Among these 500 tweets, we manually identified 75 with a matching \CR check. Workers correctly matched 63/75 tweets %at least one worker correctly matched 
according to our ground truth, while the baseline method choosing the highest SentenceBERT score correctly matched 59/75 tweets.
%The workers matched 54/75 tweets according to our ground truth, which shows an acceptable accuracy. 
After running the study over the 5322 tweets, we obtain 2208 tweets (3043 notes) matching with \CR checks. 
%As some \CR checks have different wording but the same meaning, we used SentenceBERT to group similar ones. %We arrive at 2208 tweets. 
An example of a tweet matching a \CR check is shown in Figure~\ref{fig:bw_example} (A,E). More examples of matched tweets, \BW notes, and \CR checks are in Table~\ref{tab:examples}. Our dataset containing matched tweets to \CR checks alongside labels from \BW and \CR \cam{ and code relevant to the paper are} available at \url{https://github.com/MhmdSaiid/BirdWatch}.}
%To assess the agreement between annotators, we compute the Krippendorff's $\alpha$ measure~\cite{Krippendorff2011ComputingKA, finegranedRoitero,roitero2020can}.
%, which is a popular measure to compute agreement between users~\cite{
%After running the study over the 500 tweets, we are left with 145 tweets matching with the \CR fact-checks, having a Krippendorff's $\alpha$ of 0.46. As certain \CR fact-checks verify very similar claims, participants matched a tweet to different \CR fact-checks with similar meaning. After intervening to merge the similar \CR data, we obtain a Krippendorff's alpha of 0.76. The final dataset contains 145 tweets matched with \CR data. An example of a tweet matching a \CR is shown in Figure~\ref{fig:bw_example} (A,E). More examples of matched tweets, \BW notes, and \CR fact-checks are in Table~\ref{tab:examples}. Our dataset containing matched tweets to \CR fact-checks alongside labels from \BW and \CR is available at [anonymized].



\subsection{Topics}
\label{subsec:topics}
We analyze how \BW notes \rev{and \CR checks compare in terms of covered topics}. We use \textit{BertTopic}, a topic-modeling technique that utilizes transformers and TF-IDF for clustering~\cite{grootendorst2020bertopic}, %run the model on our data and 
to predict the topic of every \BW tweet and \CR \rev{claim} for the year 2021 and report their frequency distributions in Figure ~\ref{fig:2021_topics}.
\textit{Politics} and \textit{Health} have high counts in both. Topic \textit{Country}, which includes news about countries all over the world, has higher counts for \CR data since \BW is deployed in the US only. \BW notes cover mostly tweets in English and is biased towards US related news, whereas the \CR data contains fact-checks in different languages and from local fact-checking agency, thus explaining the high number of country-related tweets. 

%As a significant fraction of our matched data is skewed towards political tweets, we repeat the matching procedure between \BW tweets and \CR fact-checks to ensure that results are consistent on a bigger sample of non-political tweets. We manually label 160 tweets against \CR fact-checks and obtain a dataset of 25 additional matched tweets (bringing the total to 170) with an inter-annotator agreement of $\alpha=0.855$.



==> BirdWatch analysis/intro.tex <==
\section{Introduction}
\label{sec:introduction}
The spread of online misinformation carries risks for the democratic process and for a decrease in public trust towards authoritative sources of news \cite{starbird2019disinformation}. %It has also become a source of noise for search engines aiming at retrieving and providing their users with reliable information \cite{clarke2020overview}.
% Given the sheer volume of misinformation online, the need to fact-check claims online and to verify their veracity becomes critical. However, fact checking at scale is challenging due to the need for expert human fact-checkers to perform a forensic process to identify and validate different sources of information to check each claim. 
% 
Fact-checking is one of the prominent solutions in fighting online misinformation. However, traditional fact-checking is a process requiring scarce expert human resources, and thus does not scale well to social media because of the continuous flow of new content \cite{hassan2015quest}. Automated methods and crowdsourcing have been proposed to tackle this challenge \cite{thorne2018automated,nakov2021automated,roitero2020can}, as they can scale with a smaller cost, but have always been studied in controlled environments. 
% 
Current approaches focus either on fully automated machine learning methods \cite{wei-etal-2019-modeling,Liu2018EarlyDO} or on hybrid human-machine approaches making use of crowdsourcing to scale-up human annotation efforts \cite{10.1145/3340531.3412048}.


The first large-scale effort of crowdsourced fact-checking was piloted by Twitter with the \BW program on the 23rd of January 2021~\cite{BWPublish}. \BW adopts a community-driven approach for fact-checking by allowing selected Twitter users to identify fallacious information by (i) classifying tweets as misleading or not, accompanied by a written review, and by (ii) classifying reviews of other \BW users as being helpful or not.
% 
In this setting, any user can create a \textit{note} for a tweet (providing some metadata about the annotations) and other users can up/down \textit{rate} such note. Multiple users can check the same content independently.
%

In this study, we perform an analysis of how crowdsourced fact-checking works in practice when compared with human experts and automated fact-checking methods.
% Aside from crowd knowledge, we take into consideration claim verifications generated by computational methods, as well as by expert fact-checkers.
To this end, we perform an analysis of the grass-root fact-checking process in \BW, including which content is selected to be fact-checked, which sources of evidence are used, and the fact-checking outcome. We also look at possible bias in terms of volume and topics as compared to experts.
To enable a fair comparison across the three fact-checking approaches (i.e., computational methods, crowd, experts), we collected a dataset of \rev{11.9k tweets with \BW checks and identified 2.2k tweets verified} both by \BW users and expert journalists. This dataset enables us to analyze and contrast the three approaches across the main dimensions in the standard fact-checking pipeline (see Figure \ref{fig:overview}). We focus on the following research questions:

\vspace{1ex}
\noindent \textbf{RQ1} How are check-worthy claims  selected by \BW users? Can %\BW users 
the crowd identify check-worthy claims before experts do? %Can experts fact-check a tweet before it even occurs?


\vspace{1ex}
\noindent \textbf{RQ2} What sources of information are used to support a fact-checking decision in \BW and how reliable are they? Does the crowd always rely on data previously fact-checked by experts, or can they be considered as ``independent fact-checkers''?

\vspace{1ex}
\noindent \textbf{RQ3} Are crowd workers able to reliably assess the veracity of a tweet? Is their assessment always considered helpful by others?

\begin{figure*}[t]
%\hspace{-2ex}
\includegraphics[scale=0.53]{images/Birdwatch2.png}
\caption{Given input tweets, the three alternative checking methods \rev{(automatic, crowd, professional checkers)} are analyzed across their comparable dimensions according to a standard fact-checking pipeline.}
\label{fig:overview}
\end{figure*}

\vspace{1ex}
Our results reveal insights from real data to answer these questions. As automatic methods are still not competitive for checking the truthfulness of online content, we focus %our attention 
on how the crowd can fact-check claims and the way they do it as compared to experts. The main contribution of this work is %therefore 
an in-depth data-driven study of how crowdsourced fact-checking can work in practice, as compared to expert fact-checking over a number of dimensions such as topics, sources of evidence, timeliness, and effectiveness.

\vspace{1ex}
\textbf{Claim Selection.} The first step in the process is deciding which claims, out of the very many produced on Twitter, should be fact-checked. This is similar to the process of assessing relevance in a search task, as users are looking for a piece of content that is valuable and that satisfies their requirements (e.g., an information need or potential harm caused by the piece of content if misleading). Regarding the selection of the claims to check, we show that the crowd mostly matches the claims selected by expert fact-checkers in terms of topics, and it is not strongly influenced by properties of the social network, such as popularity of tweets. 
Moreover, we analyze the responsiveness of crowd and experts with respect to fresh tweets and found that in some cases the crowd is orders of magnitude faster in generating a correct fact-checking outcome.



\vspace{1ex}
\textbf{Evidence Retrieval.} In terms of sources, \BW users and fact-checkers rely on different set of online resources, with only few reference websites in common. For the  sources used by the crowd and the experts, we also compare the quality perceived by the \BW community against the quality ratings obtained  from a professional journalistic tool. The two scoring methods show correlation, but also remarkable bias in source quality assessment by the crowd on some topics related to politics.

\vspace{1ex}
\textbf{Claim Verification.}
In terms of effectiveness of the claim verification, we show that crowdsourcing may be an effective checking strategy in most settings, even comparable to the results obtained by human experts, but does not lead to consistent, actionable results for some topics. 
We also analyze the agreement among \BW users and the use of different scoring functions to aggregate their feedback, including the one used in production by Twitter.

\vspace{1ex}
Our observations show how crowdsourcing fact-checking in practice can bring an added value as compared to expert fact-checkers or computational methods used in isolation. Additionally, we release the first dataset of tweets with labels from expert fact-checker, crowd, and computational methods.


In the rest of the paper, we discuss related work in fact-checking and crowdsourcing (Section~\ref{sec:relatedWork}), introduce the datasets collected and crafted for our study (Section~\ref{sec:data}), and discuss the empirical results for our analysis (Section~\ref{sec:results}). Finally, we discuss the main challenges and opportunities for crowdsourced fact-checking %starting from our observations
(Section~\ref{sec:discussion}) and conclude the paper with some open research questions (Section~\ref{sec:conclusion}).



% OLD:



% \paolo{FIRST paragraph: fact checking and how it is important and why it cannot scale with experts.}
% \gd{not AI, but talk about how the crowd can play a role in the different steps of the fact-checking pipeline}
% \paolo{SECOND: crowdsourcing and AI tools are coming to help, but they have not been tested in real setting. \BW gives us data to evaluate and sometimes it works, sometimes if fails}.
% Several papers study crowd-sourced fact checking, but how effective is it ``in the wild''? The \BW initiative provides us data to evaluate the effectiveness of this effort over multiple dimensions.


% \paolo{THIRD: Experts are good and expensive, crowd is cheaper but not accurate. Given some textual content, it would be great to assign the claims to verify correctly. But how do we do that? this is different from related tasks in the pipeline, such as stance detection and it's hard, as a claim can be difficult to check for the crowd for multiple reasons}.

% \paolo{FOURTH: we create the first dataset of tweet ids that are manually characterized wrt how clearly that can be labelled as true or false. For this characterization we use signals coming from real Tweets and their verification done by fact checkers and experts (via claim reviews). From this dataset, we design the first model to classify the textual claims as hard/easy to verify}

% Our key contributions are the following:
% \begin{itemize}
    % \item the first dataset of tweets characterized by how clearly their claims can be labelled as true or false with crowdsourced judgements and linked ground truth from fact-checkers;\mohammed{do we want to release the matched dataset? If so, we should mention that it contains some subjectivity.}
    % \item an analysis of the grass-root fact checking process in \BW and its selection bias in terms of volume, topics, and \gd{political orientation} \mohammed{Check slides about pipeline}
    % \item an analysis of what makes a tweet hard to be fact checked by the crowd\mohammed{maybe also if we can find a tweet fact-checked by the crowd but not the experts, where the crowd does not use links to snopes/poynter. We might even look at the unmatched dataset.} and a supervised model to predict if a tweet would lead to high levels of disagreement about its veracity.\mohammed{to discuss}
    
% \end{itemize}


% In the following,
% we set the stage by giving the background information;
% we report our analysis of the crowdsourced fact checking done by \BW users, exposing the cases where it works and when it fails compared to the decisions for the same claims by expert checkers;
% the analysis leads to creation of new dataset of Tweets annotated with the difficulty in checking them; finally, we report the first ML model that tackles this problem.














==> BirdWatch analysis/results.tex <==
% \begin{figure}[t]
% %\hspace{-2ex}
% \includegraphics[scale=0.40]{topic_heatmap.png}
% \caption{Correlation Heatmap of \BW and \CR time series per t   opic.}
% \label{fig:HeatMapTopic}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.4]{images/CheckWorth.png}
%     \caption{Claim check-worthiness score of \BW tweets and \CR fact-checks.}
%     \label{fig:checkWorth}
% \end{figure}



% \begin{figure}[t]
% %\hspace{-2ex}
% \includegraphics[scale=0.65]{images/NG_BW_boxplot.png}
% \caption{Box plot of journalist scores and \BW labels.}
% \label{fig:BoxPlotSources}
% \end{figure}





% \begin{figure}[t]
% %\hspace{-2ex}
% \includegraphics[scale=0.5]{images/BwCrNgKDE.png}
% \caption{Stacked Density Plots of scores of \BW and \CR links. }
% \label{fig:KDEPlotSources}
% \end{figure}





\section{Results}
\label{sec:results}
We report results in addressing our three research questions next.
%in each of the following subsections.

\subsection{RQ1: Claim Selection}
\label{subsec:rq1}
We analyze how \BW participants effectively identify check-worthy claims in a comparison with fact-checking experts.
%by analyzing trends on a per-topic basis. 
We also compare \BW users, who do not necessarily have journalistic training, against computational methods for this task.
%when it comes to claim check-worthiness.

\subsubsection{Topic Analysis} After predicting the topic of every \BW tweet and \CR fact-check, we plot the frequency distribution of four topics showing interesting trends, on a monthly basis, in Figure~\ref{fig:TopicPlot}. The high count of \BW tweets and \CR fact-checks covering political tweets show that they both consider the \textit{Politics} topic important. The similar trends for this topic suggest that both methods react similarly to news and major events in terms of claim selection. For example, 
the peak in \textit{Politics} for both methods in August is related to the Taliban take-over of Afghanistan. 
%\CR fact-checks was related to the conflict in the Gaza Strip in May.
We observe the same trend for the topics \textit{Economy} and \textit{Natural Disasters}. 

However, for the  \textit{Health} related tweets, we observe an abrupt change in the trends from July 2021. This is due to the emergence of the COVID-19 Delta variant in US, which triggered more tweets about the topic, mainly discussing masks/vaccines issues, and more \BW notes on this topic. 
This is accompanied by a decrease in the number of health-related fact-checks, which can be explained by multiple reasons. 
%One is the increase of the political fact-checks of the same month due to Taliban take-over of Afghanistan. 
One explanation is that the most important issues about masks and vaccines had already been debunked before the Delta variant. This shows that \rev{despite} fact-checks are available online, numerous social network users keep spreading false claims that have previously been debunked (see also Section \ref{subsec:ClaimVerif}). 

%Finally, t
Topic selection also reflects the different geographic focus of the two methods. For example, the \BW peak in February in topic \textit{Economy} is due to the Texas power crisis, %which is 
a US-specific event.
\rev{Despite the differences, our results show that both \BW participants and \CR experts pick the content to verify in response to the events happening in reality, independently from the specific topic.}


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.44]{images/BoxPlots2.png}
    \caption{(A) shows a box plot of claim check-worthiness scores of \BW tweets and \rev{the claims in the} \CR fact-checks. (B) shows a box plot of journalist scores compared to the final verdict of \BW users \rev{(x-axis)}.}
    \label{fig:BoxPlots}
\end{figure}

\subsubsection{Computational Methods} We report on the ClaimBuster API for claim check-worthiness~\cite{HassanALT17}. Given a sentence, the API provides a score between 0.0 and 1.0, where a higher score indicates that the sentence contains check-worthy claims. We run the API on \BW tweets and \rev{the claims in the} \CR fact-checks, with the associated box plots for the scores in Figure~\ref{fig:BoxPlots} (A). \rev{The results show a check-worthiness median score at around 0.4, for both sets of claims, while in ClaimBuster the suggested threshold for check-worthiness is 0.5~\cite{HassanALT17}. One explanation of the difficulties of computational methods for claim selection is the bias in the training data used to build them. Indeed, most available datasets for this task are of high-quality text, coming from articles or political speeches, while the text used on Twitter is usually much noisier, e.g., due to the use of slang}.


\begin{figure}
    \centering
    \includegraphics[scale=0.41]{images/popularity.png}
    \caption{Tweet popularity and \BW activity.}
    \label{fig:pop}
\end{figure}

\subsubsection{Tweet Popularity}
We check whether the claim selection process of \BW users is affected by the popularity of a tweet. For every tweet, we retrieve the number of retweets and favorites and sum them to obtain a quantifiable popularity score. As expected, Figure~\ref{fig:pop} shows that popular tweets receive more activity than others from the \BW community, i.e., have more notes and ratings. However, there are popular tweets with low \BW activity and unpopular tweets with high number of notes and ratings. 

%\mohammed{not sure is we should add numbers about how many of these tweets are retweets of more popular tweets.}   


\subsubsection{Temporal Analysis} We analyze tweets (T), \BW notes (B), and \CR fact-checks (C) time-wise. As a note can only occur after a tweet, we have three different configurations: (i) Tweet occurs first, then \BW note, then \CR fact-check (TBC), (ii) Tweet then \CR fact-check then \BW note (TCB), and (iii) \CR fact then Tweet then \BW note (CTB).

\textbf{TBC:} There are \rev{129/2208} tweets in our matched data for this case. In all tweets, \BW users provide a response much faster than experts. On average, a \BW provides a response 10X faster than an expert. These examples show how \BW participants can fact-check claims with reliable sources without the need of \CR fact-checks such as ID \#4 in Table~\ref{tab:examples}.

\textbf{TCB:} In our dataset, a \CR rarely occurs after a tweet and before a \BW. We observe faster responses from \CR than \BW users for \rev{26/2208} tweets.  Since the granularity of the \CR is days while that of \BW is seconds, there are also \rev{17/2208} tweets that occur on the same day, and we cannot state which of the two was actually faster. 
%However, it is likely that although these tweets got `late' notes from \BW users, there are other tweets that are similar and got faster \BW notes\mohammed{not sure we could verify this easily...}.

\textbf{CTB:} The majority of the matched tweets follow this pattern, with most of them related to US politics and COVID-19. As Twitter is an open space, several users tend to spread false news even after they have been fact-checked, specifically those related to Trump winning the elections. We discuss more this issue in Section~\ref{sec:discussion}.


\vspace{1ex}
{\emph{Claim Selection Take-away Message:}} \BW users and \CR experts show correlation in claim selection decisions w.r.t. major news and events, but with important differences due to the circulation of claims that have been already debunked by experts.  The crowd seems to be effective also in identifying tweets with misleading claims even before they get fact-checked by an expert.
Also, both popular and non-popular tweets get verified by \BW users.
\rev{Computing} the check-worthiness of a tweet does not lead to effective results using current \cam{off the shelf APIs}.%methods.


\subsection{RQ2: Evidence Retrieval}
Both crowd checkers and experts report the sources used in their verification process.
We analyze such sources and then contrast their quality according to an external journalistic tool. 

\subsubsection{Descriptive Statistics}

We extract all links from \BW notes. We find a total of 12,909 links covering  2,014 domains. Unsurprisingly, the top cited links are those coming from journalistic and fact-checking sites (Politifact, Reuters, NYtimes) and governmental websites, such as USGS and CDC. The distribution of the links is right-skewed, where half of the links are from only 29 domains.
\CR checks contain 76,769 links covering only 73 domains of fact-checking groups and journalists. The distribution of links shows less skewness than that of \BW.
%since the used links are concentrated in fewer domains.

%\noindent{\textbf{Intersection.}} We observe that 
\BW participants use only 17 domains in common to those of the \CR experts. The other 56 \CR domains, which are not in the overlap, include 53 
%not included, probably since \BW launched only for U.S., while the domains are of 
local resources, such as news outlets, for non US countries as fact-checking organizations work at a global scale and \BW focuses on US.  
\BW sources are a larger number as they range from Wikipedia and YouTube videos to medical websites and research papers.



\subsubsection{Expert Judgement of Source Quality}
\label{sec:sourceQuality}
We compare ratings of source quality of \BW users to those of expert fact-checkers.
To assess the quality of web sources, we rely on an external tool that provides a score (between 0 and 100) where the higher the score, the higher the quality of the source\footnote{\url{https://www.newsguardtech.com}}. The score is obtained by journalists manually reviewing every website, and we refer to it as the \textit{journalist score}.

For every note in our matched dataset, we first compute a \BW score indicating whether the links are high-quality sources or not by performing a majority voting on the ratings of the note, and we then compute the average journalist score of every link in the note. \cam{Out of 3043 notes, 2231 contained links. We obtained results for \rev{656}, while the others either had (i) no ratings (363/2231), (ii) no journalist scores (698/2231), (iii) nor both (309/2231), or (iv) there was no majority in the ranking votes (205/2231).
}
%either (i) \cam{had ratings and links in the notes, but} did not have a journalist score \rev{(807/3043)}, (ii) did not have ratings (\rev{1484/3043}), or (iii) there was no majority in the ranking votes (\rev{96/3043}).


%had a conflict between the ratings where there was a 50/50 split. 



A box plot of journalist scores and \BW labels is shown in Figure~\ref{fig:BoxPlots} (B). For note links rated as high-quality by \BW users (with majority voting), we observe high journalist scores. The majority of tweets of the notes are related to US elections \rev{and COVID-19}, with \BW users citing sources such as Politifact and \rev{CDC}. \rev{Some sources in the notes have been classified as being high-quality by \BW users but low-quality w.r.t. the journalist scores. Those notes share mainly COVID-19 studies such as Mayoclinic.org, a nonprofit American medical center, and fda.gov, the US food and drug administration, that are regarded as reliable sources in the US but do not meet all the requirements for high journalist score.}


% \begin{table*}[]
%     \centering
%     \begin{tabular}{p{4cm}|p{8cm}|p{1cm}|p{2cm}}
%     %\toprule\\
%          \textbf{Tweet}&\textbf{Note}&\textbf{NG}&\textbf{BW}  \\
%          \midrule\\
%          \texttt{Joe Biden is President In Name Only. \#PINO} &
%         \texttt{Biden is the President of the United States.   (\textbf{Link1}) (\textbf{Link2})  Ellis worked with Rudy Giuliani to overturn the 2020 election.} &
%         Link1 :100/100  Link2: 95/100 &
%         12/14 rated as unreliable sources.\\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

%A considerable number of sources 
\cam{238/656 notes contain sources that are \rev{rated as low-quality}, but have a high journalist score.} These notes are debunking news about US politics, specifically about Trump winning the 2020 elections \rev{and misinformed COVID-19 content}. These tweets include links to reliable sources, but a significant fraction of \BW users labeled such links as low-quality. This shows how some \BW users convey partisanship, forming a group of people trying to deceive the \BW program to serve their common interest, such as supporting a political party in social media.

Such groups can be effective in ``gaming'' the algorithm~\cite{EpsteinPR20}, ultimately having a profound effect on \BW since (i) the biased \BW participants can steer the ultimate label of a note to their favor, thus spreading misinformation, and (ii) by increasing their weight in the \BW platform since if one's ratings match those of the ultimate rating, they will get a higher weight. \cam{As an example, for the tweet \texttt{`Joe Biden is President In Name Only. \#PINO'}, a certain note replied that Biden is indeed the president with links from \textit{Politifact} and \textit{APNews}, both having journalistic scores of 100/100 and 95/100 respectively while 12/14 of the raters identified such sources as unreliable. }

We also compute journalist scores for links in \BW and \CR data. As \BW users use many links, we only computed scores for the top-100 occurring links that form 68.6\% of the data. While both distributions of \BW and \CR link scores attain a median of 1.0, links by \CR fact-checks have lower variance with a minimum of 0.875, while that of \BW notes is 0.495.
%The results in Figure~\ref{fig:KDEPlotSources} show that, as expected, links used by experts have always high scores while scores used by \BW users vary by their score.

\vspace{1ex}{\emph{Evidence Retrieval Take-away Message:}} Expert fact-checkers rely on a relatively small set of high-quality sources to verify claims, while \BW participants provide a variety of sources that seem to be neglected by fact-checkers. While most of these sources are evaluated as credible (by journalists) and useful (by the \BW crowd), malicious users might game the algorithm and effectively label notes as unhelpful according to their ideology. % and beliefs.
%label the links as non-trustworthy and down vote the note, thus rendering the note unhelpful.


\begin{figure}[t]
\includegraphics[scale=0.35]{images/ClassSplit.png}
\caption{Violin Plot of note counts and class splits of the classification labels of notes. The figure shows the Kernel Density Estimation (KDE) plot of every note count, with their respective data points. Tweets with two notes are dominant, with most notes agreeing on the label. Other note counts do show full agreement on the label (0/100), with more cases of disagreement as the number of notes increase.}
\label{fig:ViolinPlotClass}
\end{figure}

\subsection{RQ3: Claim Verification}
\label{subsec:ClaimVerif}
We ponder whether \BW participants provide accurate judgements. We first compare agreement (i) among themselves and then (ii) with \CR expert fact-checkers. We then analyze different scoring functions for note aggregation, and finally \rev{report results for computational methods.}
%study the temporal relationships between notes and fact-checks.




\subsubsection{Internal Agreement}
\label{subsubsec:internal}
We use the participants' classification labels to see whether the tweet is classified as misinformed or not.
To compute agreement, we use the standard metrics Krippendorff’s alpha~\cite{Krippendorff2011ComputingKA} and Fleiss's kappa~\cite{Fleiss1971MeasuringNS}. However, due to the large sparsity in the data and the huge number of missing values, both metrics fail to provide meaningful results \cite{checco2017let}. We then compute the variance as a metric for agreement. Lower variance means that all \BW participants agree on the classification label.  

A violin plot is shown in Figure~\ref{fig:ViolinPlotClass} for tweets with various note counts.
On the y-axis, we report the density of the class splits, where a class 0/100 indicates full agreement across the users and 50/50 indicates full disagreement.
We see that most tweets have two notes and the majority of users perfectly agree on the final classification label. The same applies to tweets with more note counts, where most of the notes agree on the final label, with conflicts happening on some tweets but with a small subset with full disagreement. A topic analysis of tweets shows that 48.3\% of tweets with full disagreement are related to either politics or COVID-19. 

% \begin{table}[t]
% \begin{tabular}{clcc}
% \toprule
% \multicolumn{1}{l}{}                   &                          &
% \multicolumn{4}{c}`{\textbf{BirdWatch}}                                                             \\
% \toprule
% %\multicolumn{2}{c}{\textbf{Tweets}} & \multicolumn{2}{c}{\textbf{Notes}}\\
% \multicolumn{1}{l}{}                   &                          & \multicolumn{1}{c}{\textbf{MM}} & \multicolumn{1}{c}{\textbf{NM}} \\
% \midrule
% \multirow{4}{1.3cm}{\textbf{Claim Review}} & \textbf{credible}        & 9 (5)                                                          & 4 (1)                                   \\
%                                       & \textbf{not\_credible}   & 149 (118)                                                          & 2 (1)                                  \\
%                                       & \textbf{not\_verifiable} & 15 (14)                                                           & 0 (0)                                  \\
%                                       & \textbf{uncertain}                & 9 (5)                                                            & 1 (1)    \\
% \bottomrule
% \end{tabular}
% \caption{Matching between \BW notes and \CR data. Number of matched tweets shown in parenthesis.}
% \label{tab:extAgr}
% \end{table}

\begin{table}
\setlength{\tabcolsep}{.445em}
\begin{tabular}{cccclccc}
\toprule
\multicolumn{1}{l}{}                                                             &
\multicolumn{1}{l}{}          & \multicolumn{5}{c}{\textbf{BirdWatch}}                                                          \\
\midrule
\multicolumn{1}{l}{\textbf{}}                                                    & \textbf{}                     & \multicolumn{2}{c}{\textbf{Notes}}            &           & \multicolumn{3}{c}{\textbf{Tweets}} \\
\midrule
\multicolumn{1}{l}{}                                                             & \multicolumn{1}{l}{\textbf{}} & \multicolumn{1}{l}{\textbf{MM}} & \textbf{NM} & \textbf{} & \textbf{MM}      & \textbf{NM}  &\textbf{Tie}    \\
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Claim\\ Review\end{tabular}}} & \textbf{credible}             & 209                               & \textbf{25}           &           & 126                & \textbf{9}    &9            \\

                                                                                 & \textbf{mostly\_credible}        & 56                             & \textbf{14}           &           & 44              & \textbf{7}  &5              \\
                                                                                 
                                                                                 & \textbf{not\_credible}        & \textbf{1983}                             & 184           &           & \textbf{1476}              & 62  & 55              \\
                                                                                 
                                                                                 & \textbf{not\_verifiable}      & 300                              & 25           &           & 225               & 8   &9             \\
                                                                                 
                                                                                 & \textbf{uncertain}            & 225                               & 22           &           & 156                & 8  &9      \\
\bottomrule
\end{tabular}
\caption{Matching the classification labels across \BW and \CR on the note level and the tweet level (obtained through majority voting). Agreement in bold.}
\label{tab:extAgr}
%\vspace{-2ex}
\end{table}

% \begin{table}[t]
% \begin{tabular}{clcc}
% \toprule
% \multicolumn{1}{l}{}                   &                          &
% \multicolumn{2}{c}{\textbf{BirdWatch}}                                                             \\
% \toprule
% \multicolumn{1}{l}{}                   &                          & \multicolumn{1}{l}{\textbf{MM}} & \multicolumn{1}{p{1cm}}{\textbf{NM}} \\
% \midrule
% \multirow{4}{1.3cm}{\textbf{Claim Review}} & \textbf{credible}        & 5                                                            & 1                                   \\
%                                       & \textbf{not\_credible}   & 118                                                          & 1                                   \\
%                                       & \textbf{not\_verifiable} & 14                                                           & 0                                   \\
%                                       & \textbf{uncertain}                & 5                                                            & 1    \\
% \bottomrule
% \end{tabular}
% \caption{Matching between \BW tweet and \CR data \mohammed{combine two tables}}
% \label{tab:extAgr2}
% \end{table}


% \begin{table*}[t]
%     \small
%     \begin{tabular}{l p{4cm} p{4cm} p{4cm} p{4cm}}
%          \toprule
%          \textbf{ID}&\textbf{Tweet}&\textbf{Note}&\textbf{Claim Review}&\textbf{Comment}  \\
%          \toprule
%          \#1&\texttt{Pregnant women, please don't take this vaccine. https://t.co/4KKlnMIbl7}&\texttt{Updated CDC guidance, and newly accepted and reviewed medical research, has stated there are no safety concerns for pregnant women to be vaccinated against COVID-19.    1. \url{https://www.nejm.org/doi/full/10.1056/nejmoa2104983}  2. \url{https://www.reuters.com/business/healthcare-pharmaceuticals/cdc-recommends-pregnant-women-get-covid-19-vaccine-2021-08-11/}}&\texttt{The vaccine is not safe for pregnant women or women planning on becoming pregnant within a few months of taking the vaccine... We are the lab rats.}&The \BW user provides proof of why the claim is False. The fetched fact-check has a label of being not credible.\\
%          \midrule
%          \#2&\texttt{The mass shooting at Marjory Stoneman Douglas High School in Parkland, Florida was real and not staged.}&\texttt{That this continues to be debated is astounding.  Yes, this really happened.  Here is a link:    \url{https://en.m.wikipedia.org/wiki/Stoneman\_Douglas\_High\_School\_shooting}}& \texttt{Say David Hogg is a crisis actor.}& The \BW note confirms what the tweet is stating, thus the label was not misleading. The \CR fact-check was stating a claim opposite to that of the tweet, and its label is not credible. \\
%          \midrule
%          \#3&\texttt{Chicago PD Says Enhanced Vid Shows Gun in 13-Year-Old Adam Toledo's Hand \url{https://t.co/B0Twu733RL}}&\texttt{Chicago Mayor Lori Lightfoot said Adam Toledo had a gun in his hand when he was fatally shot by a police officer, or words to that effect.}&\texttt{Adam Toledo did not have the gun in his hand when he was approached by the police who shot him. He has his arms up and complied. The gun was on the floor, not his hands.}& There is a difference in granularity of claim.\\
%          \midrule
%          \#4&& && .\\
%     \end{tabular}
%     \caption{Examples of \BW Notes and \CR facts.}
%     \label{tab:examples}
% \end{table*}

\setttsize{\Small}

\begin{table*}[t]
\small
\resizebox{0.99\textwidth}{0.255\textheight}{
\begin{tabular}{lp{3.1cm} p{4.2cm}cp{3.5cm}l p{3.9cm}}
\hline
\textbf{ID}  & \textbf{Tweet}      & \multicolumn{2}{c}{\textbf{BW Note}}               & \multicolumn{2}{c}{\textbf{CR Fact}} & \textbf{Comment}   \\ \cline{3-6}
    &                      & \multicolumn{1}{l}{\textbf{Text}} & \multicolumn{1}{l}{\textbf{Label}} & \textbf{Text}    & \textbf{Label}    &                    \\ \hline
\multicolumn{1}{c}{\textbf{\#1}} & \texttt{Pregnant women, please don't take this vaccine. \url{https://t.co/4KKlnMIbl7}} &\texttt{Updated CDC guidance, and newly accepted and reviewed medical research, has stated there are no safety concerns for pregnant women to be vaccinated against COVID-19.} \emph{(links omitted for brevity)}
% 1. \url{https://www.nejm.org/doi/full/10.1056/nejmoa2104983}  2. \url{https://www.reuters.com/business/healthcare-pharmaceuticals/cdc-recommends-pregnant-women-get-covid-19-vaccine-2021-08-11/}}                            
& MM                             & \texttt{The vaccine is not safe for pregnant women or women planning on becoming pregnant within a few months of taking the vaccine... We are the lab rats.}        & NC          & The \BW user provides proof of why the claim is False. The fetched fact-check has a label of being not credible. \\
\midrule

\textbf{\#2}&\texttt{The mass shooting at Marjory Stoneman Douglas High School in Parkland, Florida was real and not staged.}&\texttt{That this continues to be debated is astounding.  Yes, this really happened.  Here is a link:    \url{https://en.m.wikipedia.org/wiki/Stoneman\_Douglas\_High\_School\_shooting}}&NM& \texttt{Say David Hogg is a crisis actor.}&NC&BW note confirms the tweet, thus the label was not misleading. The CR check states a claim opposite to the tweet and its label is not credible.\\
\midrule
\textbf{\#3}&\texttt{Chicago PD Says Enhanced Vid Shows Gun in 13-Year-Old Adam Toledo's Hand \url{https://t.co/B0Twu733RL}}&\texttt{Chicago Mayor Lori Lightfoot said Adam Toledo had a gun in his hand when he was fatally shot by a police officer, or words to that effect.}&MM&\texttt{Adam Toledo did not have the gun in his hand when he was approached by the police who shot him. He has his arms up and complied. The gun was on the floor, not his hands.}&CR&Difference in granularity of the claim. For CR check, the claim is whether Toledo was holding a gun; while for the BW note, the claim was whether Chicago's mayor \textit{said} that Toledo hold a gun.\\
\midrule
\textbf{\#4}& \texttt{New poll indicates Biden approval at 11\%. The LOWEST approval rating of ANY president in American history. ~Gallup via Daily Caller}&\url{https://fivethirtyeight.com/features/how-were-tracking-joe-bidens-approval-rating/}&MM&\texttt{Biden approval at 11\%}&NC&The \BW participant provided a reliable source (score of 92.5) 7 days before a fact-check by an expert was available.\\
\midrule
\textbf{\#5}& \texttt{Biden thinks he came to the US Senate 120 years ago?!?}&\texttt{US President Joe Biden made a clear joke at his first press briefing since his inauguration, in which he said he went to the Senate 120 years ago. This is a self-deprecating joke and shouldn't be taken seriously.} %, as nobody alive today was around 120 years ago.}
&MM&\texttt{Joe Biden said, `With regard to the filibuster, I believe we should go back to the position of the filibuster that existed just when I came to the United States Senate 120 years ago.'}&CR&The Tweeter took a joke seriously, which was interpreted as misleading by the \BW participant.\\
\bottomrule
\end{tabular}}
\caption{Examples of Tweets, \BW Notes, and matched \CR fact-checks. \BW uses labels misleading/potentially misinformed (MM) or not misleading (NM), while \CR uses credible (CR) or not credible (NC).}
\label{tab:examples}
%\vspace{-2ex}
\end{table*}


\subsubsection{External Agreement}
\label{subsubsec:external}
After matching \BW data with \CR fact-checks, we compare their labels. Table~\ref{tab:extAgr} shows that the majority of \CR labels match the \BW ones. Specifically, in terms of notes, there are \rev{2022 cases (25+14+1983)} where they agree and \rev{449 cases} of disagreement. In terms of tweets, there are \rev{1492 (9+7+1476) decisions with the same classification label and 232 (126+44+62) with different labels. For 69 (9+5+55) tweets there is a tie in the voting across \BW users.} For completeness, we report also the numbers for other \CR labels (`not\_verifiable' and `uncertain'), even if they have no  mapping to \BW classification labels. 
%however, note that mapping from them to \BW labels is not trivial.    %especially those that were labelled as misleading. 
%This also shows that \BW users do verify claims that are considered check-worthy by expert fact-checkers. 
\rev{We did some analysis to understand the cases where the labels are not aligned, some examples are reported in Table~\ref{tab:examples}.
Among the 209 notes that are labeled as credible by the \CR fact-checks and misinformed by the \BW participants, the most common cause are texts with multiple claims, % because of %. Five out of these nine notes have 
%granularity problems,
i.e., multiple facts are reported in a tweet %. For example, there are multiple claims in the tweet 
and the fact-checked claims differ (ID \#3). In other cases, tweets are mistakenly labelled as misinformed, e.g., because a joke is taken seriously by a Twitter user (ID \#5). Finally, assuming correct \CR labels, we believe in some cases the mismatch is due to biased \BW users. For the tweets labeled as not credible by \CR fact-checks and not misleading by \BW notes, we observe cases where a \BW note is the negated version of the \CR fact-check (ID \#2), thus producing opposite labels. There are also mismatch of labels, even though the \BW user provides evidence from a link that has a high journalistic score (0.875).}

\subsubsection{Note Helpfulness Score}
In the real-world production setting, not all \BW notes are used for finding the ultimate label that gets exposed on the platform. In fact, a \textit{note helpfulness score} is computed by the platform for each note, and those having a high enough score are used for computing the ultimate label. \BW exposes the code for computing such score, however, the public code does not include raters' scores into consideration. We use the available code and filter out notes that are not helpful for the final label, using a Twitter-defined threshold for the note helpfulness score (0.84). We are left with \rev{533 tweets (over 2208)} that pass the threshold, \rev{with 333 notes labeling the tweets according to \CR checks. About 95\% of notes label the tweets as misleading, thus} 
%All of those notes correctly label the tweets as misleading. 
%We observe an increase in the accuracy of the classification label, w.r.t. the experts, from the simple majority voting at the expense of the coverage.
%, i.e., no tweets labeled as not misleading. 
indicating that \BW users tend to rate misleading tweets more than non-misleading ones, in agreement with previous work~\cite{Prollochs2021CommunityBasedFO}. Of course, malicious ratings of the classification labels can steer the note helpfulness score in misleading directions, similarly to the judgement for source quality as discussed in Section~\ref{sec:sourceQuality}.

\subsubsection{Computational Methods.} We compare our matched data with labels coming from computational fact-checking systems. We use again ClaimBuster, \rev{as it can also verify claims}~\cite{HassanZACJGHJKN17}, and E-BART~\cite{BrandRSD21}.
ClaimBuster provides correct results for \rev{118 out of 2208 tweets, where 2090 tweets have no output from the model with an F1-score of 0.042. E-BART correctly labels 369 (over 2208) and does not produce a decision for 59 tweets with an F1-score of 0.17. A random classifier produces an average F1-score of 0.333 with 0.008 standard deviation.} As for claim selection, tweets are harder to handle for computational methods than news articles and quotes from politicians, which are the bulk of content in training corpora.

\vspace{1ex}
{\emph{Claim Verification Take-away Message}}: \BW users show high enough levels of agreement to reach decisions in the vast majority of cases. The \BW crowd focuses mostly on misleading tweets and shows high agreement with expert fact-checkers in terms of classification label. %, i.e., \BW users can scale more with misinformation than expert fact-checkers.
Computational methods have room for improvement in automatically verifying tweets.

% Topics of tweets
% Time Analysis:
    %TBC: can be faster and reach conclusion with different results, mostly agree on claims checked
    %TCB: not common
    %CTB:repeated tweets

% \mohammed{probably we do the exps on (1) the entire dataset and (2) the enitre dataset - trump-related tweets  }
% Dimensions over the notes, most of those apply also for analysis of the ratings:
% \begin{enumerate}
%     \item accuracy wrt ground truth provided by professional fact checkers. We will link notes with claim reviews - notice that annotation will require some human verification (label T/F the top 10 matches for every tweet).\mohammed{regarding the matching, if the crowd uses poynter/snopes links, do we disregard them?}
%     \item accuracy wrt computational methods. Here the risk is that most computational methods will fail. However, this is an interesting observation to report over a novel real dataset and it would be nice to compare the effectiveness of workers vs methods.\mohammed{Do we want to use smth like the FEVER baseline?}
%     \item agreement among workers: disagreement on ratings vs disagreement on notes on the same tweet \mohammed{check slides}
%     \item summary analysis:
%     \begin{itemize}
%         \item NLP analysis of summary (e.g., length/quality)
%         \item estimate URL/source reliability (start by fetching content of links in summary)
%         \item correlate checkboxes with summary
%         \item correlate assessment quality (wrt ground truth) and evidence provided
%     \end{itemize}
%     \item effect of aggregation functions over user votes/ratings
%     \item effect of scales transformations (?)
%     \item (missing: workers background / bias)
% \end{enumerate} 


% Questions: 
% \begin{enumerate}
%     \item do the checkers debunk worth-checking tweets?
%     \item are the checks effective in debunking the tweets? 
%     \item are the votes effective in championing the good checks?
% \end{enumerate}

% \subsection{Checkers analysis}
% \mohammed{We can maybe try to do a simple analysis on the birdwatch users. Although we do not have access to their accounts, we can maybe analyze what notes they like/dislike and classify them accordingly. For example, a user who upvotes all pro-trump related tweets is pro-trump. We can make use of the topic model we have.}
% Dimensions over the checkers: 
% \begin{enumerate}
%     \item check submitted 
%     \item check voted
%     \item network of participant ids
%     \item estimate participant reliability score (from data itself vs from ground truth)
%     \item profiling participants and do aggregation to get a final label for every tweet (based on combination of notes and ratings)
%     \item \mohammed{Analyze 'Author Helpfulness Score'}
%     \item \mohammed{Analyze 'Rater Helpfulness Score'}
% \end{enumerate}


% Questions: 

% \mohammed{We need to agree on what "worthy\-checking" is.}
% \begin{enumerate}
%     \item do the checkers debunk worth-checking tweets?
%     \item are the checks effective in debunking the tweets? 
%     \item are the votes effective in championing the good checks?
%     \item \mohammed{What birdwatch data columns are helpful in debunking/verifying a tweet? If we can label the data suing the matching, we can run a simple random forest model on the data and see which columns are more important..}
% \end{enumerate}


% More dimensions \paolo{to be checked against lists above}
% \begin{enumerate}
%     \item NLP analysis of note summaries
%     \begin{itemize}
%         \item length 
%         \item toxic language detection
%         \item propaganda language detection
%         \item stance detection?
%         \item quality of text measures (get baseline methods for this task: https://nyu-mll.github.io/CoLA/)
%     \end{itemize}
%     \item analysis of the links in summaries
%     \begin{itemize}
%         \item expand links
%         \item analyze Web sources (open ended, to decide how)
%         \item see if their trust of the link correlates with external sources
%     \end{itemize}
%     \item collect more tweet info
%     \begin{itemize}
%         \item profile of the author, number of followers, tweets
%         \item retweet, likes, comments for the tweet
%         \item topic modeling (LDA version for short texts - GSTM?) [also for summaries?] - try simple clustering if this fails
%     \end{itemize}
%     \item execute more computational fact checking methods on the claims (Fever pipeline?)
% \end{enumerate}


% \section{Discussion}
%\mohammed{this would be a more manual analysis.}

%\subsection{A New Dataset}

